MPISE: Symbolic Execution of MPI Programs

Message Passing Interfaces (MPI) plays an important role in parallel computing. Many parallel applications are implemented as MPI programs. The existing methods of bug detection for MPI programs have the shortage of providing both input and non-determinism coverage, leading to missed bugs. In this paper, we employ symbolic execution to ensure the input coverage, and propose an on-the-fly schedule algorithm to reduce the interleaving explorations for non-determinism coverage, while ensuring the soundness and completeness. We have implemented our approach as a tool, called MPISE, which can automatically detect the deadlock and runtime bugs in MPI programs. The results of the experiments on benchmark programs and real world MPI programs indicate that MPISE finds bugs effectively and efficiently. In addition, our tool also provides diagnostic information and replay mechanism to help understanding bugs.

==> ack.tex <==
\section{Acknowledgment}
We would like to thank the authors of Cloud9 and KLEE for the wonderful platform. Especially Stefan Bucur, for his useful suggestions.


==> mpiklee-lastest - extended/abs.tex <==
% !TEX root = main.tex
%--------------------------------------------
%
\begin{abstract}
Message Passing Interfaces (MPI) plays an important role in parallel computing. Many parallel applications are implemented as MPI programs. The existing methods of bug detection for MPI programs have the shortage of providing both input and non-determinism coverage, leading to missed bugs. In this paper, we employ symbolic execution to ensure the input coverage, and propose an on-the-fly schedule algorithm to reduce the interleaving explorations for non-determinism coverage, while ensuring the soundness and completeness. We have implemented our approach as a tool, called \mpise{}, which can automatically detect the deadlock and runtime bugs in MPI programs. The results of the experiments on benchmark programs and real world MPI programs indicate that \mpise{} finds bugs effectively and efficiently. In addition, our tool also provides diagnostic information and replay mechanism to help understanding  bugs.
\end{abstract}


==> mpiklee-lastest - extended/ack.tex <==
\section{Acknowledgment}
We would like to thank the authors of Cloud9 and KLEE for the wonderful platform. Especially Stefan Bucur, for his useful suggestions.


==> mpiklee-lastest - extended/conclusion.tex <==
% !TEX root = main.tex
%--------------------------------------------
%
\section{Conclusion}
\label{sec:conclusion}

MPI plays a significant role in parallel programming. To improve the reliability of the softwares implemented using MPI, we propose \mpise{} in this paper to use symbolic execution to analyze MPI programs, targeting to find the bugs of an MPI program automatically. Existing work on analyzing MPI programs suffers problems in different aspects, such as scalability, feasibility and input or non-determinism coverage.
%
%%%%%%%%%%%%%%
We employ symbolic execution to tackle the input coverage problem, and propose an on-the-fly algorithm to reduce the interleaving explorations for non-determinism coverage, while ensuring the soundness and completeness.
%
%To attack the lack of both input coverage and coverage over the space of nondeterminism of the testing and some formal verification methods, we proposed our method which includes a scheduling algorithm to avoid naively explore all possible interleaving, namely canonical schedule, and a way to treat wildcard receive named lazy matching. We also discussed the soundness and completeness of our on-the-fly schedule and lazy matching.
We have implemented a prototype of \mpise{} as an adoption of Cloud9, and conducted extensive experiments. The experimental results show that \mpise{} can find bugs effectively and efficiently. \mpise{} also provides diagnostic information and utilities to help people understand a bug.

For future work, there are several aspects. In one aspect, we plan to support non-blocking MPI operations, which are widely used in nowadays MPI programs. In another aspect, we want to refine our MPI model further, \emph{e.g.}, using a more realistic library, to improve the precision of symbolic execution. Finally, we are also concerned with improving the scalability of \mpise{} and the analysis of production-level MPI programs.


==> mpiklee-lastest - extended/exp.tex <==
% !TEX root = main.tex
\section{Implementation and Experiments}
\label{Sec: Experiments}

\subsection{Implementation}
We have implemented our approach as a tool, called \mpise{}, based on Cloud9 \cite{Bucur:2011:PSE:1966445.1966463}, which is a distributed symbolic executor for C programs. Cloud9 enhances KLEE \cite{Cadar:2008:KUA:1855741.1855756} by enabling the support of most POSIX interfaces and parallelism. The architecture of \mpise{} is shown in Fig \ref{fig:arch}.
%And the workflow is displayed in Figure \ref{fig:arch}.
\vspace{-2mm}
\begin{figure}[!htpb]
\vspace{-2mm}
  \centering
  \includegraphics[width=0.8\textwidth]{arch.pdf}\\
  \caption{The architecture of \mpise{}. }\label{fig:arch}
  \vspace{-3mm}
\end{figure}

The target MPI programs written in C is fed into LLVM-GCC compiler to obtain the LLVM bytecode, which will be linked with a pre-compiled library, \emph{i.e.}, TOMPI \cite{Demaine97athreads-only}, as well as the POSIX runtime library. Then, the linked executable program will be symbolically executed. Basically, TOMPI is a platform that uses multi-threads to simulate the running of an MPI program. TOMPI provides a subset of MPI interfaces, which contains all the MPI APIs we consider in this paper. An MPI program can be compiled and linked with TOMPI libraries to generate a multi-thread executable, which is supposed to generate the same output as that of the parallel running of the MPI program. Hence, we use TOMPI %instead of real MPI platforms, such as MPICH2 or OpenMPI,
as the underlying MPI library. By using TOMPI, we can use the support for concurrency in Cloud9 to explore the path space of an MPI program run with a specific number of processes. When a path ends or a deadlock is detected, \mpise{} records all the information of the path, including the input, the orders of message passings, \emph{etc}. For each path, we generate a corresponding test case, based on which one can use \emph{replayer} to reproduce a concrete path.
%Note that the TOMPI library is instrumented manually, all the concerned APIs are hooked to trigger signals to
%\mpise{}. \mpise{} symbolic execute the linked bytecode, exploring the interleaving with the help of the scheduler.
%reports the result of checking deadlock and runtime failure and produces a test case,
%With the test case, one can use the replayer to reproduce the results.
Compared with Cloud9, our implementation of \mpise{} consists of the following new features:

\begin{itemize}
\item \textbf{New scheduler.} Cloud9 employs a none-preemptive scheduler, \emph{i.e.}, a process would keep being executed until it gives up, such as encountering an explicit preemption call or process exit.
Clearly, we need a new scheduler for \mpise{}. We have implemented our on-the-fly scheduler that can schedule the MPI processes according to the algorithms in Sections \ref{sub:sched} \& \ref{section:wr}.
\item \textbf{Environment support for MPI APIs.} Cloud9 does not ``recognize" MPI operations, while \mpise{} makes the symbolic engine know MPI operations based on TOMPI, including MPI\_Send, MPI\_Ssend, MPI\_Recv, MPI\_Barrier, \emph{etc}. The message passing APIs are dealt specially for scheduling, while other MPI APIs are treated as normal function callings.
\item \textbf{Enhanced Replay.} \mpise{} can replay each generated test case of an MPI program, which can help user to diagnosis bugs such as deadlock and assertion failure. The replayer of \mpise{} extends the replayer component of Cloud9 by using the on-the-fly schedule when replaying a test case. During replaying, the replayer uses the recorded input to feed the program, and follows the recorded schedules to schedule the processes.
\item \textbf{Enhanced POSIX model.} \mpise{} heavily depends on the library models it uses. However, the POSIX model provided by Cloud9 is not sufficient for us to symbolically execute MPI programs. The reason is we need to maintain a process specific data area for each process when symbolically executing each process. Because we use multi-thread programs to simulate the behaviour of MPI programs, we have improved the mechanism for multi-thread programs in Cloud9 to support maintaining thread specific data.
\end{itemize}

\subsection{Experimental evaluation}\label{subSec:ee}

We have conducted extensive experiments to validate the effectiveness and scalability of \mpise{}. All the experiments were conducted on a Linux server with 32 cores and 250 GB memory.

Using \mpise{} to analyze the programs in the Umpire test suite \cite{ppopp-VakkalankaSGK08},
%in which each test case is an input-independent program.
we have successfully analyzed 33 programs, \emph{i.e.}, either no deadlock detected or detecting a deadlock as expected.

The Umpire test case are input-independent, \emph{i.e.} the inputs have nothing to do with whether a deadlock happens. Hence, we conduct the experiments on the programs with input-dependent deadlocks. The conducted test cases mainly cover two typical situations of deadlock \cite{CPE:CPE701}: point-to-point ones and collective ones. Point-to-point deadlocks are usually caused by (1). a send/receive routine has no corresponding receive/send routine; (2). a send-receive cycle may exist due to the improper usage of send and receive. Collective deadlocks are typically caused by (1). missed collective routines (such as Barrier); (2). improper ordering of some point-to-point or/and collective routines.


In our experiments, we also use ISP and TASS to analyze the programs. Fig \ref{fig:er} displays the experimental results, including those of ISP and TASS.

\begin{figure}[!htpb]
  \centering
{\small
 \begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
 &Program & \multicolumn{2}{|c|}{ISP} & \multicolumn{2}{|c|}{TASS} & \multicolumn{2}{|c|}{\mpise{}}\\
 \cline{3-8}
 & & Result & Time(s) & Result & Time(s) & Result & Time(s)\\
 \hline
 & anysrc-deadlock.c & Deadlock & 0.126 & Fail & 1.299 & Deadlock & 1.59\\
 \cline{2-8}
 & basic-deadlock.c & Deadlock & 0.022 & Fail & 1.227 & Deadlock & 1.46\\
 \cline{2-8}
 Input& collect-misorder.c & Deadlock & 0.022 & Fail & 0.424 & Deadlock & 1.48\\
 \cline{2-8}
 Indep-& waitall-deadlock.c & Deadlock & 0.024 & Fail & 1.349 & Deadlock & 1.49\\
 \cline{2-8}
 endent& bcast-deadlock.c & Deadlock & 0.021 & Fail & 0.493 & Deadlock & 1.40\\
 \cline{2-8}
 & complex-deadlock.c & Deadlock & 0.023 & Fail & 1.323 & Deadlock & 1.46\\
 \cline{2-8}
 & waitall-deadlock2.c & Deadlock & 0.024 & Fail & 1.349 & Deadlock & 1.48\\
 \hline
% & cond-barrier-deadlock.c & No & 0.060 & Fail & 0.858 & Deadlock & 11.29\\
% \cline{2-8}
% & cond-head-to-head.c & No & 0.021 & Fail & 1.537 & Deadlock & 12.36\\
% \cline{2-8}
% Input& cond-rr-deadlock.c & No & 0.021 & Fail & 1.212 & Deadlock & 12.26\\
% \cline{2-8}
% Depe-& cond-recv-any-deadlock.c & No & 0.021 & Deadlock & 1.674 & Deadlock & 12.60\\
% \cline{2-8}
% ndent&cond-bcast.c&No&0.021&No&1.433&Deadlock&11.39\\
% \cline{2-8}
% &cond-collect-misorder.c&No&0.023&Deadlock&1.505&Deadlock&14.52\\
% \cline{2-8}
% &cond-waitall-deadlock.c&No&0.102&Fail&1.284&Deadlock&14.32\\
 & barrier-deadlock.c & No & 0.061 & Fail & 0.863 & Deadlock & 1.71\\
 \cline{2-8}
 & head-to-head.c & No & 0.022 & Fail & 1.542 & Deadlock & 1.67\\
 \cline{2-8}
 Input& rr-deadlock.c & No & 0.022 & Fail & 1.244 & Deadlock & 1.67\\
 \cline{2-8}
 Depe-& recv-any-deadlock.c & No & 0.022 & Deadlock & 1.705 & Deadlock & 1.70\\
 \cline{2-8}
 ndent&cond-bcast.c&No&0.021&No&1.410&Deadlock&1.63\\
 \cline{2-8}
 &collect-misorder.c&No&0.023&Deadlock&1.682&Deadlock&1.85\\
 \cline{2-8}
 &waitall-deadlock3.c&No&0.104&Fail&1.314&Deadlock&1.78\\
 \hline
 \end{tabular}
}
\caption{Experimental results}\label{fig:er}
\vspace{-4mm}
\end{figure}
In Fig \ref{fig:er}, we divide the experimental results into two categories: input independent programs and input dependent ones. For each category, we select programs that can deadlock caused by different reasons, including  head to head receive, wait all, receive any, \emph{etc}. For each input dependent program, we generate the input randomly when analyzing the program with ISP, and analyze the program for 10 times, expecting to detect a deadlock. The execution time of analyzing each input dependent program with ISP is the average time of the 10 times of runnings. According to the experimental results, we can conclude as follows:
%\begin{itemize}

\mpise{} can detect the deadlock in all the programs. ISP misses the deadlock for all the input dependent programs. TASS fails to analyze most of programs. Thus, \mpise{} outperforms ISP and TASS for all the programs in Fig \ref{fig:er}. The reason is, \mpise{} uses symbolic execution to have an input coverage guarantee, and the scheduling algorithms ensures that any deadlock caused by the MPI operations considered in this paper will not be missed. In addition, we utilize TOMPI and Cloud9 to provide a better environment support for analyzing MPI programs. The reason of the common failure of TASS is that TASS does not support many  APIs, such as \emph{fflush}(stdout) of POSIX and MPI\_Get\_Processor\_Name of MPI, and needs manually modifying the analyzed programs.

For each program, the analysis time using \mpise{} is longer than that of using ISP or TASS. The reason is two fold: firstly, we need to symbolically execute the bytecodes including those of the underlying MPI library, \emph{i.e.}, TOMPI. For example, for the input dependent program cond-barrier-deadlock.c, the number of the executed instructions is 302625.  Secondly, the time used by \mpise{} includes the linking time of the target program byte code and TOMPI library.  In addition, we need to record states and do solving during symbolic execution, which also needs more time than dynamic analysis.

For the rest programs in Umpire test suite, \mpise{} either reports a deadlock that actually does not exist or aborts during symbolic execution. The reason is we only consider the synchronous communications in MPI programs, or some advanced MPI operations, such as MPI\_Type\_vector, are not supported by \mpise{}. The improvement with respect to these aspects is our future work.
%Another 10 tests gets different results either because \mpise{} treats Recv as blocking, or because TOMPI treats Send as synchronous send. This would bring deadlocks that should not happen when running with a more complex library which do not simply treats all send as synchronous, \emph{i.e.} the reported deadlock also happens when one run the TOMPI-linked-program.

%The remaining 31 tests aborts during symbolic execution, since these tests used MPI operations such as MPI\_Type\_vector that TOMPI do not support, \mpise{} treats these as external calls and aborts the run when these unmodeled functions are encountered.

\begin{figure}[!h]
\vspace{-2mm}
  \centering
\subfigure[Instruction count of CPI]{
\label{fig:cpi:ins}
\includegraphics[width=0.45\textwidth]{cpi_instruction.pdf}}
\hspace{-0.1em}
\subfigure[Symbolic execution time of CPI]{
\label{fig:cpi:time} %% label for second subfigure
\includegraphics[width=0.4\textwidth]{cpi_time.pdf}}
  \centering
\subfigure[Instruction count of DT]{
\label{fig:dt:ins}
\includegraphics[width=0.45\textwidth]{dt_sym_instruction.pdf}}
\hspace{-0.1em}
\subfigure[Symbolic execution time of DT]{
\label{fig:dt:time} %% label for second subfigure
\includegraphics[width=0.4\textwidth]{dt_sym_time.pdf}}
\subfigure[Instruction count of IS]{
\label{fig:is:ins}
\includegraphics[width=0.45\textwidth]{IS_instruction_blue.pdf}}
\hspace{-0.1em}
\subfigure[Symbolic execution time of IS]{
\label{fig:is:time} %% label for second subfigure
\includegraphics[width=0.4\textwidth]{IS_time_blue.pdf}}
\caption{The experimental results under different numbers of processes}
\label{fig:realworld}
\vspace{-5mm}
\end{figure}

To validate the scalability of \mpise{}, we use \mpise{} to analyze three real world MPI programs, including an MPI program (CPI) for calculating $\pi$ and two C MPI programs (DT and IS) from NSA Parallel Benchmarks (NPB) 3.3 \cite{NPB} with class S. The LOC of DT is 1.2K, and the program needs an input that is either BH, WH or SH for showing the communication graph name. IS is an MPI program for integer sorting, and the LOC of IS is 1.4K. \mpise{} can analyze these three programs successfully, and no deadlock is found. We make the input symbolic and symbolically execute all the three MPI programs under different numbers of parallel processes. The experimental results are displayed Fig \ref{fig:realworld}. Because IS can only be run with $2^n$ ($n \ge 1$) processes, we do not have results for the case of 6 processes.

From Fig \ref{fig:realworld}, we can observe that, for all the three programs, the number of the executed instructions and the symbolic execution time do not increase exponentially with respect to the number of processes. It justifies that \mpise{} avoids the exponential increasing of instructions or symbolic execution time caused by the parallelism by the on-the-fly scheduling algorithms. Note that we make the input of DT symbolic ones, and this program aborts early when fed with input BH and the process number that is less than 12,  this explains the sudden rise of both analyze time and instructions when the number of processes goes from 10 to 12 in Fig.\ref{fig:dt:ins} and Fig.\ref{fig:dt:time}.












==> mpiklee-lastest - extended/intro.tex <==
% !TEX root = main.tex
%------------------------------------
%
\section{Introduction}
\label{sec:intro}
In the past decades, Message Passing Interface (MPI) \cite{MPI2.2} has become the \emph{de facto} standard programming model for parallel programs, especially in the filed of high performance computing. A significant part of parallel programs were written using MPI, and many of them are developed in dozens of person-years \cite{Gopalakrishnan:2011:FAM:2043174.2043194}.

Currently, the developers of MPI programs usually use traditional methods to improve the confidence of the programs, such as traditional testing and debugging \cite{GDB}\cite{DDT}. In practice, developers may waste a lot of time in testing, but only a small part of behavior of the program is explored. MPI programs have the common features of concurrent systems, including non-determinism, possibility of deadlock, \emph{etc}. These features make the shortage of testing in coverage guarantee more severe. Usually, an MPI program will be run as several individual processes. The nature of non-determinism makes the result of an MPI program depend on the execution order of the statements in different processes. That is to say, an MPI program may behave differently with a same input on different executions. Hence, sometimes it is harder to find the bugs in an MPI program by a specific program execution.

To improve the reliability of MPI programs, many techniques have been proposed. Basically, we can divide the existing work into two categories: static analysis methods \cite{MPISPIN}\cite{TASS}\cite{Strout:2006:DAM:1156433.1157634} and dynamic analysis methods \cite{Vo:2010:SDD:1884643.1884681} \cite{cav08-isp}. A static method analyzes an MPI program without actually running it. The analysis can be carried out on code level \cite{TASS} or model level \cite{MPISPIN}. Usually, a static method needs to make an abstraction of the MPI program under analysis \cite{MPISPIN}\cite{Strout:2006:DAM:1156433.1157634}. Therefore, many static methods suffer the false alarm problem.

Dynamic methods, such as testing  and runtime verification, need to run the analyzed MPI programs and utilize the runtime information to do correctness checking \cite{KrammerBMR03}\cite{ita}\cite{conf/sc/VetterS00}, online verification \cite{ppopp-VakkalankaSGK08}\cite{Vo:2010:SDD:1884643.1884681}, debugging \cite{DDT}\cite{TotalView}, \emph{etc}. Traditional testing methods work efficiently in practice by checking the correctness of a run under a given test harness. However, testing methods cannot guarantee the coverage on non-determinism even after many runs of a same program input. Other dynamic analysis methods, such as ISP \cite{ppopp-VakkalankaSGK08},  provide the coverage guarantee over the space of non-determinism and scale well, but they are still limited to program inputs. While TASS \cite{TASS} employs symbolic execution and model checking to verify MPI programs, it only works on small programs due to the limited support of runtime library models.

In this paper, we use symbolic execution to reason about all the inputs and try to guarantee the coverage on both input and non-determinism. We symbolically execute the statements in each process of an MPI program to find input-related bugs, especially runtime errors and deadlocks. For the non-determinism brought by the concurrent features, we use an on-the-fly scheduler to reduce the state space to be explored in the analysis, while ensuring the soundness and completeness. Specially, to handle the non-determinism resulted from the wildcard receives in MPI programs, we dynamically match the source of a wildcard receive into all the possible specific sources in a \emph{lazy} style, which avoids the problem of missing bugs. Furthermore, unlike the symbolic execution plus model checking method in \cite{TASS}, which uses an MPI model to simulate the runtime behaviors of MPI library, we use a true MPI library as the model, which enables us to analyze real-world MPI programs.

To summarize, our paper has the following main contributions: firstly, we propose an on-the-fly scheduling algorithm, which can reduce unnecessary interleaving explorations while ensuring the soundness and completeness; secondly, when attacking the non-determinism caused by wildcard receives, we propose a technique, called lazy matching, to avoid blindly matching each process as the source of a wildcard receive, which may lead to false positives; finally, we have implemented our approach in a tool called \mpise{}, and conducted extensive experiments to justify its effectiveness and efficiency in finding bugs in MPI programs.

The rest of this paper is organized as follows. Section 2 introduces the back- ground and shows the basic idea of \mpise{} by motivating examples. Section 3 describes the details of the algorithms implemented in \mpise{}. Section 4 explains our implementation based on Cloud9 and shows the experimental results. Finally, Sections 5 discusses the related work and the conclusion is drawn in Section 6.
%\vspace{-4mm}

==> mpiklee-lastest - extended/mpiklee.tex <==
% !TEX root = main.tex
\section{Symbolic execution algorithms}
%In this section, we introduce the notion of transition systems to model MPI programs and present a scheduling algorithm to avoid exploring all possible interleaving. Furthermore, to attack non-determinism brought by wildcard receive,  we combined it with our lazy matching algorithm, which could help to explore all possible matches of wildcard receives, hence a guarantee over the space of non-determinism is provided.
In this section, we will introduce a general framework for symbolic execution of MPI programs first, and then present a scheduling algorithm during the symbolic execution. Furthermore, to attack the non-determinism brought by wildcard receives, we will present a refined scheduling method, which can ensure the exploration of all the possible matches of a wildcard receive.

%\subsection{Models of MPI Programs}
%\label{sub:model}


%
% However, this directed graph omits the scheduling process. We introduce the idea of ``dependent chain" here: a dependent chain is a series of processes and MPI operations of the form $$\dots P_i\overset{OP_{ik}}{\hookrightarrow} P_j \dots, OP\in \{S, R, B\}$$ which means that $P_i$ is either sending or receiving a message or waiting for $P_j$ for a barrier, $OP_{ik}$ says that this is the kth MPI operation of $P_i$.
%
% A dependent chain changes with scheduling: when the current process firstly comes to $P_0$, the chain becomes $P_0\overset{OP_{01}}{\hookrightarrow} P_{dest(OP)}$, where $dest(OP)$ is the destination process rank if $OP \in \{S,R\}$ and $P_1$ if $OP = B$.

% A dependent chain always start from $P_0$, and has limited length (the length of a dependent chain is the number of MPI operations of the chain). The dependent chain changes from time to time: when a unmatched MPI operation is encountered, the length of the chain grows by 1 while a matched MPI operation is encountered, the length of the chain decreases by 1 if the operation is an S or R.

%We focus on deadlock reachability problem of transition systems. A global state is deadlocked if it has no compositional action enabled, and it is not a final state.
%}
To start with, we introduce some notions first. When symbolically executing a sequential program, the symbolic executor keeps tracking of states, each of which consists of a map that records the symbolic/concrete value of each variable, a program counter and a path condition. For an MPI program, a state during symbolic execution is composed by the states of the parallel processes. A state $s'$ is said to be the successor of a state $s$, if $s'$ can be obtained by symbolically executing a statement in one process. With the notion of \emph{state}, we define a \emph{deadlock} to be the state that has no successor, and at which there is at least one process that does not terminate. Recall that symbolic execution will do state forking when encountering a branch statement. For MPI programs, in addition to branch statements, the concurrency nature can also result in state forking. Theoretically, for the current state, if there are more than one process, say $n$,  that can be executed, there are $n$ possible successor states. Hence, besides the number of branch statements, the number of parallel processes also makes the path space increase exponentially. Algorithm \ref{alg:framework} presents a general framework for symbolic execution of MPI programs.

%Since an MPI program typically involves a fixed number of processes created at inception, its state consist
%\hspace{0.1em}
%\vspace{1mm}
{\small
\begin{algorithm}[H]
Search($MP$, $n$, $slist$)\{\\
$Active=\{P_0, \dots, P_n\}$ ; $Inactive = \emptyset$\;
NextProcCandidate= -1; worklist = \{initial state\}\;
\While{\emph{(}worklist is not empty\emph{)}}
{
$s$ = pick next state\;
$p$ = \emph{Scheduler}($s$)\;
\If{$p \neq null$}{
$stmt$ = the next statement of $p$\;
%\If{l is non-MPI operations}
%{
%perform symbolic execution\;
%}
%\Else
%{
%\tcc{Treat MPI calls specially.}
%\emph{sempi}($s,l$);
%}
SE($s$, $p$, $stmt$);
}
}
\}
\caption{Symbolic Execution Framework}\label{alg:framework}
\end{algorithm}
}%\vspace{1mm}

Basically, the symbolic execution procedure is a worklist-based algorithm. The input consists of an MPI program, the number of the parallel running processes and the symbolic variables. At the beginning, only the initial state, \emph{i.e.}, composed by the initial states of all the processes, is contained in the worklist. Then, new states can be derived from the current state and put into the worklist. State exploration is done if there is no state in the worklist. Because of state forking, we usually have a way for space exploration, such as depth first search (DFS) and breadth first search (BFS). Clearly, it is hard or even impossible to explore the whole path space. In fact, for the state forking introduced by the concurrent feature, sometimes there is no need to add all the possible successor states to the worklist, which can still capture the behavior of the program precisely in our context. Hence, different from the usual symbolic execution algorithm, in our algorithm, we first select a state from worklist (Line 5, where a search algorithm can be used), then we make a decision (Line 6, the details of which will be given in Section \ref{sub:sched}) of which process is scheduled for symbolic execution. Finally, we symbolically execute the next statement of the scheduled process, in which some new states may be generated.

Basically, for the non-communication statements in an MPI program, the symbolic execution semantics is same as usual. In the following of this section, we will concentrate on explaining the scheduling of the processes and the handling of the communication operations.
\vspace{-4mm}
\subsection{On-the-fly scheduling}
\label{sub:sched}

With the general framework in Algorithm \ref{alg:framework}, we introduce our scheduler here, aiming to avoid naively exploring the interleavings of all the processes.
For each process of an MPI program during symbolic execution, the process is \emph{active} if it is not asleep. Usually, we make a process asleep when the process needs to communicate but the corresponding process is not ready, whose details will be given in Algorithm \ref{alg:se}. We maintain the current status of each process via two sets: $Active$ and $Inactive$. At beginning, all the processes are contained in $Active$. If a process is made to be asleep, it will be removed from $Active$ and added to $Inactive$. Because we schedule the processes on-the-fly, we use a global variable $NextProcCandidate$ to denote the index of the next process to symbolically execute. The following \mbox{Algorithm \ref{alg:scheduler}} gives how to do scheduling.

\vspace{2mm}
{\small
\begin{algorithm}[H]
Scheduler(s)\{\\
\If{$NextProcCandidate != -1$ and $Proc_{NextProcCandidate}$ is active}
{
$Next = NextProcCandidate$\;
$NextProcCandidate = -1$\;
\Return $Proc_{Next}$\;
}
\ElseIf{$Active \neq \emptyset$}{
\Return the process $p'$ with the smallest rank in $Active$\;
}
\If {$Inactive \neq \emptyset $}  {Report Deadlock\; }
\}
\caption{Scheduling the Next Process for Symbolic Execution}\label{alg:scheduler}
\end{algorithm}
}\vspace{2mm}

First, we check whether there is a next process that needs to be executed and is also active. If there exists one, the process identified by $NextProcCandidate$ will be selected, and the next process global variable is reset (Line 1$\sim$5); otherwise, we return the active process with the smallest rank if exists (Line 6$\sim$7). Finally, if there is no active process that can be scheduled, and the $Inactive$ set is non-empty, \emph{i.e.}, there exists at least one process that does not terminate, we report that a deadlock is found (Line 8$\sim$9).


Now, we explain how to symbolically execute each statement. In \mbox{Algorithm \ref{alg:se}}, we mainly give the handling for MPI APIs considered in this paper. The local statements in each process do not influence the other processes, and the symbolic execution of basic statements, such as assignment and branch, is the same with the traditional approach \cite{Cadar:2008:KUA:1855741.1855756}. Hence, the symbolic execution of local statements is omitted for the sake of space. In Algorithm \ref{alg:se}, Advance($S$) denotes the procedure in which the program counter of each process in $S$ will be advanced, and \mbox{Match($p$, $q$)} denotes the procedure in which the synchronization between $p$ and $q$ happens, \emph{i.e.}, the receiver receives the data sent by the sender, and the program counters of $p$ and $q$ will be both advanced.

If a $Send(dest)$ is encountered and there is a process in $Inactive$ that matches the statement, we move that process from $Inactive$ to $Active$ (Line 5) and advance the two processes (Line 6). If there is no process that can receive the message, we add this process into \emph{Inactive} set (Line 8), and switch to the destination process of the send operation (Line 9). The execution of a receive operation is similar, except that when the receive operation is a wildcard receive, we make the current process asleep (the reason will be explained in Section \ref{section:wr}).

{\small
\begin{algorithm}[H]
SE($s$, $p$, $stmt$)\{\\
\Switch{kindof\emph{(}$stmt$\emph{)}}{
\Case{Send\emph{(}dest\emph{)}}{
\If{$stmt$ has a matched process $q \in Inactive$}{
$Inactive = Inactive \setminus \{q\}$;\ $Active = Active \cup \{q\}$\;
Match($p$, $q$)\;
}
\Else{
$Inactive = Inactive \cup \{p\}$\;
$NextProcCandidate= dest$\;
}
\Return\;
}
\Case{Recv\emph{(}src\emph{)}}{
\If{src \emph{!= MPI\_ANY\_SOURCE} }{
\If{$stmt$ has a matched process $q \in Inactive$}{
$Inactive = Inactive \setminus \{q\}$;\ $Active = Active \cup \{q\}$\;
Match($p$, $q$)\;
}
\Else{
$Inactive = Inactive \cup \{p\}$\;
$NextProcCandidate = src$\;
}
}
\Else{
$Inactive = Inactive \cup \{p\}$\;
}
\Return\;
}
\Case{Barrier}{
\If{$mc_b == \emptyset$}{
$mc_b = \{P_0,\dots, P_n\} \setminus \{ p \}$\;
$Inactive = Inactive \cup \{p\}$\;
}
\Else{
$mc_b = mc_b \setminus \{p\}$\;
\If{$mc_b == \emptyset$}{
Advance($\{P_0, \dots, P_n\}$)\;
$Inactive = \emptyset$;\ $Active = \{P_0, \dots, P_n\}$\;
}
\Else{
$Inactive = Inactive \cup \{p\}$\;
}
}
\Return\;
}
\Case{Exit}
{
$Active = Active \setminus \{p\}$\;
\Return\;
}
%\Other{
%Perform ordinary symbolic execution\;
%}
}%end of switch
Advance($\{p\}$)\;
\}
\caption{Symbolic Execution of a Statement}\label{alg:se}

\end{algorithm}
}

%I think we need to define the match of two processes.
For handling barriers, we use a global variable $mc_b$ to denote the rest processes that need to reach a barrier for a synchronization. When a barrier statement is encountered, if $mc_b$ is empty, we initialize $mc_b$ to be the set containing the rest processes (Line 24) and add the current process into $Inactive$ (\mbox{Line 25}). If $mc_b$ is not empty, we remove the current process from $mc_b$. Then, if $mc_b$ is empty, \emph{i.e.}, all the processes have reached a barrier, we can advance all the processes (Line 29) and make all the processes active (Line 30); otherwise, we add the current process into \emph{Inactive} set (Line 32). When encountering an Exit statement, which means the current process terminates, we remove the current process from $Active$ (Line 35). 
%For the rest kinds of statements, we perform symbolic execution as usual and advance the current process, which we omit in the algorithm for the sake of space.

In summary, according to the two algorithms, the symbolic execution process will continue to execute the active process with the smallest rank until a preemption happens caused by an unmatched MPI operation. From a state in symbolic execution, we do not put all the possible states into the worklist, but only the states generated by the current process.   This is the reason why we call it on-the-fly scheduling. Actually, we only explore a sub space of the whole program path space, but without sacrificing the ability of finding deadlock bugs. The correctness of our on-the-fly scheduling algorithms is guaranteed by the following theorem, whose proof is given in appendix.

%when there are no matched MPI operation, \mpise{} employs non preemptive  scheduling, i.e. a process would keep being executed till it give up(sleep itself). However, when a matched MPI operation occurs, preemption happens. Hence the scheduling points in on-the-fly schedule are  explicit preemption calls and the MPI operations, either matched or unmatched. When \emph{NextProcCandidate} is set to the rank of a process, the scheduler would make it executed at next schedule, or it would come to the one with the smallest rank in $Active$. Recall that we employ on-the-fly schedule to attack the interleaving explosion problem of naively exploring. Following on-the-fly scheduling, \mpise{} actually explores only a subgraph of the whole program graph, without hurting the ability of finding each possible deadlock.
%What is it really?

\begin{theorem}\label{theorem-1}
Given a path of an MPI program from the initial state to a deadlocked state, there exists a path from the initial state to the same deadlocked state obtained by the on-the-fly scheduling. And vice versa.
\end{theorem}

\subsection{Lazy matching algorithm}\label{section:wr}

Note that so far, we do not treat wildcard receives. Actually, wildcard receives are one of the major reasons of non-determinism. Clearly, we cannot blindly rewrite a wildcard receive. For example, in Fig \ref{fig:brewrite}, if we force the wildcard receive in $Proc_1$ to receive from $Proc_2$, a deadlock will be reported, which actually will not happen. 
%The reason is that the wildcard receive expects a send from $Proc_2$ that actually does not communicate with $Proc_1$. 
In addition, if we rewrite a wildcard receive immediately when we find a possible match, we still may miss bugs. As shown in Fig \ref{fig:erewrite}, if we match the wildcard receive in $Proc_0$ with the send in $Proc_1$, the whole symbolic execution will terminate successfully, thus a deadlock, which will appear when the wildcard receive is matched with the send in $Proc_2$, is missed. %In our approach, we try to explore all the possible matches of a wildcard receive by rewriting it into each source specific receive.

\begin{figure}[!htp]
\vspace{-2mm}
  \centering
\subfigure[Blind rewriting of a wildcard receive]{
 \label{fig:brewrite}
 \begin{tabular}{c|c|c}
 \hline
  $Proc_0$          & $Proc_1$            &     $Proc_2$\\
 \hline
    Send(1)        & Recv(ANY)  &    local statements\\
 \hline
 \end{tabular}
 }
 \quad
\subfigure[Eager rewriting of a wildcard receive]{
 \label{fig:erewrite}
 \begin{tabular}{c|c|c}
 \hline
  $Proc_0$          & $Proc_1$            &     $Proc_2$\\
 \hline
  Recv(ANY) ; Recv(2)      & Send(0)   &    Send(0) \\
 \hline
 \end{tabular}
 }
 \vspace{-2mm}
\caption{Rewriting of a wildcard statement}
 \vspace{-2mm}
\end{figure}

To solve this problem, we employ a lazy style approach instead of an eager one. That is, we delay the selection of the send candidate of a wildcard receive until the whole symbolic execution procedure blocks. To be detailed, when the symbolic execution encounters a wildcard receive, we would make the current process asleep (Line 20 in Algorithm \ref{alg:se}), waiting for all possible senders. When a matched send is found, the current process will also be made asleep, and we switch to the next active process. When there is no process that can be scheduled, \emph{i.e.}, all the processes are in $Inactive$, we match the wildcard receive to each possible matched send by forking a successor state for each one. Thus, Algorithm \ref{alg:scheduler} needs to be refined to handle wildcard receives. The refined parts are given as follows.

{%\scriptsize
\small{
\begin{algorithm}[H]
Scheduler($s$)\{\\
...\\
\If {$Inactive \neq \emptyset $}  {
\If {Exists a \emph{Recv(ANY)} process in $Inactive$} {
$PS = Inactive$\;
\For{each \emph{Recv(ANY)} process $p \in Inactive$}{
\For{each matched process $q \in Inactive$ of $p$}{
$Inactive = PS \setminus \{p, q\}$;\ $Active = \{p, q\}$\;
AddState($s$, $p$, $q$)\;
}
}
\Return null\;
}
\Else{
Report Deadlock\;
}
}
\}
\caption{Refined Scheduling for Handling Wildcard Receives}\label{alg:refined-scheduler}
\end{algorithm}
}
}
\vspace{2mm}

For each process encountering a wildcard receive in $Inactive$, we add a new state for each of its matched sender processes (Line 9). The AddState($s$, $p$, $q$) denotes a procedure that does the synchronization between $p$ and $q$, advances both $p$ and $q$, and adds the new state to the worklist. Thus, we are exploring all the possible cases of a wildcard receive. If there are multiple Recv(ANY) processes, we are interleaving the matches of all the processes. The example in Fig \ref{fig:breakup} demonstrates this situation. When all the processes are asleep, if we match the Recv(ANY) in $Proc_1$ with the send in $Proc_0$ first, no deadlock will be detected; otherwise, if we match the Recv(ANY) in $Proc_2$ with the send in $Proc_3$ first, a deadlock will be detected.
\vspace{-4mm}
\begin{figure}[!htpb]
  \centering
 \begin{tabular}{l|l|l|l}
 \hline
  $Proc_0$          & $Proc_1$            &     $Proc_2$ & $Proc_3$\\
  \hline
    Send(to:1) \qquad       & Recv(from:ANY)\qquad &   Recv(from:ANY)  \qquad &Send(to:2)\\
  \hline
  & Recv(from:3)\qquad& &Send(to:1)\\
  \hline
     \end{tabular}
  \caption{Multiple wildcard receives}\label{fig:breakup}
  \vspace{-3mm}
\end{figure}

Therefore, after considering wildcard receives, the matches of different wildcard receives are not independent. We deals with this problem by naively interleaving the match orders of wildcard receives. This leads to redundant interleavings, but dose not miss interleaving-specific deadlocks. The optimization is left to our future work. The proof of correctness of our handling for wildcard receives %is ensured by the interleavings of matches and exploring all the possible matches of a wildcard receive. The proof of the correctness is provided in appendix.
is provided in appendix.


%Therefore, any deadlock in a source specific MPI program with the assumptions we set holds would be caught with our on-the-fly schedule.
%\textcolor[rgb]{1.00,0.00,0.00}{Ensured that ISP failed to discover this deadlock. And run this in mpich binary code 10 times would possibly catch this. YET i don't know whether we should point out this, if we do, how?}

%For simplicity, \mpise{} deals with this problem by naively interleaving the explore order of $SR_{*}$ global transitions who share the same father global state. This leads to redundant interleaving, but do not miss interleaving-specific deadlocks. The optimization is left to our future work.


==> mpiklee-lastest - extended/overview.tex <==
% !TEX root = main.tex
\section{Background and Motivating Example}
In this section, we briefly describe symbolic execution and the scope of the MPI APIs we are concerned with, then show how our algorithm works by motivating examples.
\subsection{Symbolic execution}
Symbolic execution \cite{K76} is a SAT/SMT based program analysis technique originally introduced in the 1970s. With the significant improvement in SAT/SMT techniques and computing power, symbolic execution draws renewed interests recently. The main idea is, rather than using concrete values, symbolic execution uses symbolic values as input values, and keeps tracking the results of numerical operations on symbolic values.
Hence, the result of a program under symbolic execution will be symbolic expressions. Most importantly, symbolic execution uses a constraint of symbolic values, called path condition (PC), to represent a path of a program. At the beginning, the path condition is \emph{true}. When encountering a branch statement, symbolic execution explores both directions of the branch. For exploring one direction, symbolic execution records (\emph{i.e.}, conjunction) the condition $cond$ corresponding to the direction in PC and queries an underlying solver with $PC\wedge cond$ to decide whether this direction is feasible. If the answer is yes, symbolic execution will continue to execute the statements following the direction, and PC is update to be $PC\wedge cond$; otherwise, it means the direction is infeasible, thus symbolic execution backtracks to the branch statement, and starts to explore the other direction. The selection of which direction of a branch to explore first can be random or according to some heuristics. Once symbolic execution reaches the end of a program, the accumulated PC represents the constraints that the inputs need to satisfy to drive the program to the explored path.
%In addition, the outputs when executing along the path also satisfy the PC.
Therefore, we can consider symbolic execution as a function that computes a set of PCs for a program. Naturally, we can use the PCs of the program to do automatic test generation \cite{Cadar:2008:KUA:1855741.1855756}\cite{Cadar:2011:SES:1985793.1985995}, bug finding \cite{Cadar:2008:KUA:1855741.1855756}\cite{godefroid2008sage}, verification \cite{xianghuadeng2006ase}, \emph{etc}.

According to the before explanation, symbolic execution is a precise program analysis technique, because each PC represents a real feasible path of the program under analysis. Therefore, when used for bug finding, symbolic execution does not suffer from the false alarm problem, and the  bugs found are real bugs. Whereas, one of the major challenge symbolic execution faces is path space exploration, which is theoretically exponential with the number the branches in the program.

%Whereas, symbolic execution faces some challenges:  one is path space exploration, which is theoretically exponential with the number the branches in the program;
%another one is constraint solving, especially when encountering the programs with complex computations, \emph{e.g.}, high order expressions, the underlying solver cannot handle the fed complex constraints.

\subsection{MPI Programs}
An MPI program is a sequential program in which some MPI APIs are used. The running of an MPI program usually consists of a number of parallel processes, say $P_0, P_1, ..., P_{n-1}$, that communicate via message passings based on MPI APIs and the supporting platform. The message passing operators we consider in this paper include:
\begin{itemize}
\item Send(dest) -send a message to $P_{dest}$ $(dest=0,\dots,n-1)$, which is the destination process of the Send operation. Note that only synchronous communications are considered in this paper, so this operation blocks until a matching receive has been posted.

\item Recv(src) -receive a message from $P_{src}$ $(src=0,\dots,n-1, ANY)$, which is the source process of the Recv operation. Note that the $src$ can take the wildcard value ``ANY", which means this Recv operation expects messages from any process. Because Send and Recv are synchronous, a Send/Recv that \emph{fails} to match with a corresponding Recv/Send would result in a \emph{deadlock}.

%which is similar to MPI\_Recv, except that Recv(src) only supports synchronous protocol, hence blocks until a matching send has been posted. Here `*' means that it can receive from any source, which we call it wildcard receive.
\item Barrier() -synchronization of all processes, which means the statements of any process should not be issued past this barrier until all the processes are synchronized. Therefor, an MPI program is expected to eventually reach such a state that all the processes reach their barrier calls. If this does not hold, there would be a deadlock.
%synchronization across all members of a group, no operations after the barrier would be posted until all of the barrier in the group are posted.
\end{itemize}

%For simplicity, we do not consider the associated buffer here, since it does not affect our algorithm. And further, we suppose that all the considered operations are blocking synchronous operations happens in a common communicator. And, no MPI\_ANY\_TAG is used, the only source of nondeterminism comes from MPI\_ANY\_SOURCE. We show few operations here for it's enough to illustrate our algorithm. Our implementation, however, covers most of the frequently-used operations.
The preceding three MPI operations are the most important operations we consider in this paper. Actually, they cover the most frequently used \emph{synchronous} communications in MPI programs.

\subsection{Motivating Examples}
 Usually, an MPI program is fed with inputs to perform a computational task, and the bugs of the program may be input-dependent. On the other side, due to the non-determinism feature, even with same inputs, one may find that bugs occur ``sometimes''.


Consider the MPI program in Fig \ref{moti-example}, if the program runs with an input that is not equal to `a', the three processes will finish normally with two matched \textrm{Send} and \textrm{Recv},
%\emph{i.e.}, $Proc_1$ receives two messages from $Proc_0$ and $Proc_2$, respectively,
as indicated by Fig \ref{fig:subfig:case1}. However, if the program is fed with the input `a', a deadlock may happen, in case that $Proc_1$ receives a message from $Proc_2$ first by a wildcard receive, and then it waits a message from $Proc_2$ and $Proc_0$ also expects $Proce_1$ to receive a message, as shown in Fig \ref{fig:subfig:case3}. Therefore, tools that do not provide input space coverage would surely fail to detect this bug if the program is not fed with `a'. Even if one is lucky enough to run the program with `a', we may still fail to detect the bug if the wildcard receive is matched with $Proc_0$, \emph{e.g.}, the case in Fig \ref{fig:subfig:case2}.
%\begin{figure}
%  \centering
% \begin{tabular}{l|l|l}
%  $Proc_0$          & $Proc_1$  & $Proc_2$          \\
%  \hline
%             &    if(x!=0) Recv(from:0) & \\
%             &     else Recv(from:*) & \\
%    Send(to:1)&Recv(from:2) & Send(to:1)\\
%   % Barrier() & Barrier() &Barrier()\\
%   \end{tabular}
%\caption{Example showing the need for both input and nondeterminism coverage}\label{moti-example}
%\end{figure}

%  if(argc != 2)
%    exit(1);

\begin{figure}[width=.9\textwidth]
\vspace{-2mm}
\begin{lstlisting}
int main(int argc, char **argv) {  	
  int x, y, myrank;
  MPI_Comm comm = MPI_COMM_WORLD;

  MPI_Init(&argc, &argv);
  MPI_Comm_rank(comm, &myrank);
  if (myrank==0) {
    x = 0;
    MPI_Ssend(&x, 1, MPI_INT, 1, 99, comm);
  }
  else if (myrank==1) {
    if(argv[1][0]!= 'a') //  argc is exactly 2
      MPI_Recv(&x, 1, MPI_INT, 0, 99, comm, NULL);
    else
      MPI_Recv(&x,1, MPI_INT, MPI_ANY_SOURCE, 99, comm, NULL);

    MPI_Recv(&y, 1, MPI_INT, 2, 99, comm, NULL);
  } else if (myrank==2){
    x = 20;
    MPI_Ssend(&x, 1, MPI_INT, 1, 99, comm);
  }
  MPI_Finalize();
  return 0;
}
\end{lstlisting}
\vspace{-4mm}
\caption{Example showing the need for both input and non-determinism coverage}\label{moti-example}
\vspace{-2mm}
\end{figure}

Thus, for detecting deadlock bugs, we need both input coverage and non-determinism coverage guarantee. The basic idea of our method is: we employ symbolic execution to cover all possible inputs, and explore all the possible matches of a wildcard receive by matching it to any possible source.

\begin{figure}[htpb]
  \centering
\subfigure[X$\neq$’a’]{
\label{fig:subfig:case1}
\includegraphics[width=0.34\textwidth]{moti-1.pdf}}
\hspace{-0.1em}
\subfigure[X==’a’ and wildcard receive matches with $Proc_0$]{
\label{fig:subfig:case2} %% label for second subfigure
\includegraphics[width=0.29\textwidth]{moti-2.pdf}}
\hspace{0.1em}
\subfigure[X==’a’ and wildcard receive matches with $Proc_2$]{
\label{fig:subfig:case3} %% label for second subfigure
\includegraphics[width=0.29\textwidth]{moti-3.pdf}}
\vspace{-1mm}
%
%\begin{minipage}[t]{0.33\linewidth}
%\centering
%\includegraphics[width=\textwidth]{ moti-1.pdf}
%\caption{argv[1][0]!=鈥檃鈥檥
%\label{fig:moti:case1}
%\end{minipage}%
%
%\begin{minipage}[t]{0.3\linewidth}
%\centering
%\includegraphics[width=\textwidth]{ moti-2.pdf}
%\caption{argv[1][0]==鈥檃鈥?and wildcard receive matches with $Proc_0$}
%\label{fig:moti:case2}
%\end{minipage}%
%
%\begin{minipage}[t]{0.3\linewidth}
%\centering
%\includegraphics[width=\textwidth]{ moti-2.pdf}
%\caption{argv[1][0]==鈥檃鈥?and wildcard receive matches with $Proc_2$}
%\label{fig:moti:case3}
%\end{minipage}%

\caption{Three cases of the program in Fig \ref{moti-example}}\label{fig:3cases}
\vspace{-2mm}
\end{figure}

To be more detailed, since we only symbolically execute one process at a time, we need to decide the exploration order of the processes. Usually, each process of an MPI program has a rank,
 %which is initialized by MPI\_Comm\_rank at the beginning and used as the identity of the process,
 we always start from the smallest ranked process and switch to another process until the current process needs synchronization, such as sending or receiving a message. Thus, the switches during symbolic execution happen \emph{on-the-fly}. Specifically, things become more complex when encountering a Recv(ANY) statement, where we need to delay the selection of the corresponding sending process until all the possible sending statements are encountered.
%Therefore, a Recv(ANY) statement will also make the current process asleep, and another executable process, if there is any, will be switched to.

For the MPI program in Fig \ref{moti-example} run in three processes, we start from $Proc_0$, \emph{i.e.}, the process with rank 0. When executing to line 9, a Send is encountered, which means a synchronization is needed. From the send statement, we know it needs to send a message to $Proc_1$. Thus, we switch to $Proc_1$ and do symbolic execution from the beginning. When the branch statement at line 12 is encountered, and $argv[1][0]$ is symbolic (we suppose it has a symbolic value $X$), the condition $X \neq{}\text{`a'}$ is added to the path condition of the true side and its negation to the false side. We mark here as a backtrack point and has two paths to follow, which are explained as follows:
\begin{description}
  \item[$X\neq{}  \text{`a'}$:] If we explore the true side first, the path condition, \emph{i.e.}, $X \neq \text{`a'}$, is fed to the solver to check the feasibility of the path. Apparently, the solver will answer yes, thus we can continue the symbolic execution of $Proc_1$. Then, Recv(0) is meet and it is exactly matched with the send in $Proc_0$. Therefore, both processes advance, and $Proc_0$ ends while $Proc_1$ goes to Recv(2). In a same manner,  $Proc_1$ gets asleep, we switch to $Proc_2$. Again the two operations matches, the whole execution will end normally, as shown in Fig \ref{fig:subfig:case1}.
  \item[$X =={} \text{`a'}$:] This side is also feasible. The symbolic execution of $Proc_1$ will encounter Recv(ANY), and switches to $Proc_2$. After executing the Send at Line 20, there is no process that can be switched to. All the possible sending processes of the Recv(ANY) in $Proc_1$ are determined. Thus, now we begin to handle the Recv(ANY) by %marking it as a backtrack point, and explore by
      matching it with each possible sending. Suppose we match the Recv(ANY) with the Send of $Proc_0$, we continue to execute $Proc_1$. We encounter another Recv at Line 17 that expects to receive a message from $Proc_2$, then $Proc_1$ and $Proc_2$ advance, and finally the whole execution ends normally, as indicated by Fig \ref{fig:subfig:case2}. On the other hand, if the Recv(ANY) is matched with the Send of $Proc_2$, when encountering the Recv in $Proc_1$, symbolic execution will switch to $Proc_2$, but $Proc_2$ has finished. Then, $Proc_0$ and $Proc_1$ can not terminated. Hence, a deadlock is detected, as shown in Fig \ref{fig:subfig:case3}.
\end{description}

In summary, the deadlock, which may happen in the program in Fig \ref{moti-example} when run in three processes, can only be encountered when the input starts with `a' and the Recv(ANY) in the second process is matched with the Send in the third process. By using our approach, \mpise{} can detect it automatically. The details of our symbolic execution algorithms will be introduced in the next section.



==> mpiklee-lastest - extended/proofs.tex <==
% !TEX root = main.tex
\newpage
\appendix
\section{Theorems and Proofs}
\label{append:models}

In order to model MPI programs, we introduce the notion of \emph{transition system} in \cite{Baier:2008:PMC:1373322}:
\begin{Definition}{Transition System}

A \emph{transition system} TS is a tuple $(S, Act,\rightarrow, I, AP, L)$, where
\begin{itemize}
\item $S$ is a set of states,
\item $Act$ is a set of actions,
\item $\rightarrow \subseteq S\times Act \times S$ is a transition relation,
\item $I\in S$ is a set of initial states,
\item $AP$ is a set of atomic propositions, and
\item $L:S\rightarrow 2^{AP}$ is a labeling function.
\end{itemize}
\end{Definition}

For an action $act$ and a state $s$, if there is a transition $\tau = \langle s, act, s'\rangle \in \rightarrow$, we say that $act$ is \emph{enabled} in state $s$, and $\tau$ is denoted as $s\overset{act}{\rightarrow} s'$. If there are no such $\tau$, $act$ is \emph{disabled} in $s$. We denote the set of actions enabled in $s$ as $enabled(s)$, \emph{i.e.}, $\{  act \mid  s_1\overset{act}{\rightarrow}s_2\wedge  s_1 = s\}$. Note that all transitions systems in this paper is assumed to be \emph{action deterministic}, \emph{i.e.} for a sate $s\in State$ and an action $\alpha \in Act$, $s$ has at most one transition labeled with $\alpha$ to another state. Hence if $\alpha\in Act$ is enabled in state $s$, we also use $\alpha(s)$ to denote the unique $\alpha$-successor of $s$, \emph{i.e.} $s\overset{\alpha}{\rightarrow}\alpha(s)$.

And we use \emph{execution} to describe the behavior of the transition system. An \emph{execution} in a transition system is an alternative sequence of states and actions $\pi = s_0\alpha_1 s_1\alpha_2\dots,\alpha_n s_n$ starts from a initial sate $s_0$ and ends at a terminal state, where $s_i\overset{\alpha_{i+1}}{\rightarrow} s_{i+1}$ holds for $ 0 \leq i < n$. We use $\lvert \pi \rvert$ to denote the \emph{length} of $\pi$, and $\lvert \pi \rvert = n$.

To model an MPI process, we define the model more precisely: $S = Loc\times Eval(Var)$ is a set of states, where $Loc$ is the locations of a process, and $Eval(Var)$ denote the set of variable evaluations that assign values to variables. $Act = \{s,r,b\}$, which means we only care about the blocking synchronous send and receive MPI operations as well as the collective operation barrier. We use $dest(op)$, where $op\in \{s,r\}$, to denote the destination of a send or a receive.

The above definition refers to only one process. However, the running of an MPI program typically consists of many processes. Therefore, we need mechanisms to provide the operational model for parallel runnings in terms of transition systems.

\begin{Definition}{Parallel composition}\\
Let $TS_{i}=(S_{i},Act_{i},\rightarrow_{i},I_{i},AP_{i},L_{i})\ i=1,2,\dots,n$ be $n$ transition systems. The transition system $TS = TS_1 \interleave_{H} TS_2 \interleave_{H} \dots \interleave_{H} TS_{n}$ is defined to be:
{$$TS = (S_1\times S_2\times \dots S_n, Act_g, \rightarrow, I_1\times I_2\times \dots I_n, AP_1\cup AP_2 \cup\dots AP_n, L_g)$$} where the transition relation $\rightarrow$ is defined by the following rule:
\begin{itemize}
\item for matched actions $\alpha,\beta \in H=\{s,r,b\}$ in distinct processes:
 $$\frac{s_i\overset{\alpha}{\rightarrow_i}s'_i \quad\wedge\quad s_j\overset{\beta}{\rightarrow_j}s'_j  \quad\wedge\quad match(\alpha, \beta)}{\langle s_1,\dots,s_i,\dots ,s_j,\dots s_n\rangle\xrightarrow{SR}{\langle s_1,\dots,s'_i,\dots ,s'_j,\dots s_n\rangle}}$$
here $match(\alpha,\beta)$ if and only if $(\alpha= s \wedge \beta=r) \vee (\alpha= r\wedge\beta= s)$, $dest(\alpha)=j$, and $dest(\beta)=i$, $SR$ is the compositional global action of s and r.

\item for matched actions $\alpha = b$ in distinct processes:
$$\frac{s_1\overset{\alpha}{\rightarrow_1}s'_1 \quad\wedge\quad \dots  s_i\overset{\alpha}{\rightarrow_i}s'_i \quad\wedge\quad \dots s_n\overset{\alpha}{\rightarrow_n}s'_n}{\langle s_1,\dots,s_i,\dots s_n\rangle\xrightarrow{B}{\langle s'_1,\dots,s'_i,\dots s'_n\rangle}}$$
Here B is the compositional global action of the local action $b$ of each process.
\end{itemize}
The labeling function is defined by $L_g(\langle s_1,\dots,s_i,\dots,s_n\rangle)= \bigcup_{1\le i\le n} L(s_i) $. And note that actions in $Act_g$ are also introduced in the above two rules.
\end{Definition}



%Given a global state $\sigma$ in a composed transition system, assume the edges coming out from $\sigma$ are $\delta_1,\dots, \delta_k$. We fix a total order on these transitions according to $min$\{ranks of  participants of $\delta\}$, \emph{i.e.}, given two SR transitions $\delta_k , \delta_k'$ where $participants(\delta_k) = \{Proc_i,Proc_j\}, i< j$ and $participants(\delta_k') = \{Proc_i',Proc_j'\}, i'< j'$, then $i < i'$  implies $k <k'$.

The composition of transition systems gives a global view of a directed graph $G=(S, \mathcal{T} )$, where the nodes in $S$ are global states and an edge in $\mathcal{T}$ is a global transition with action $SR$ or $B$. Note that the idea behind our on-the-fly schedule is that, for a global state, we only choose some of the transitions to move on and discard the others. Hence, we only explore a subgraph. To describe this subgraph, we first introduce some notions here.

Given a global state $\sigma$ in a composed transition system, we fix a total order on actions enabled in $\sigma$ according to $weight(act)$, where $act\in enabled(\sigma) , \delta = \sigma\overset{act}{\rightarrow} \sigma'$, and  $$weight(act)=\left\{
                 \begin{array}{ll}
                   1, & \hbox{if $act = B$;} \\
                   i, & \hbox{if $act = SR$ , $\sigma=\langle s_1,\dots, s_n\rangle$, $\sigma'=\langle s_1,\dots, s'_i,\dots,s'_j,\dots s_n\rangle$.}
                 \end{array}
               \right.
$$

\emph{i.e.}, $act_1 < act_2$ \textrm{iff} $weight(act_1) < weight(act_2)$. When an action $act \in enabled(s)$ has the minimal weight, we say that $act$ ranks first in $enabled(s)$.


 \begin{Definition}
 %Let $\tilde{\mathcal{T}}$ denote the set of all global transitions $\tau$ for which either $\tau$ is global barrier or $\tau$ ranks first in all the transitions begins from it's source global state. Let $\tilde{G} = (S,\tilde{\mathcal{T}})$.
Let $\tilde{G} = (S, \tilde{\mathcal{T}})$ be a subgraph of $G$, where $\tilde{\mathcal{T}}$ is defined as follows:
\[\tilde{\mathcal{T}} = \bigcup_{s\in S}\{\tau \mid \tau=\langle s, act, s'\rangle \wedge act\ \text{ranks first in}\ enabled(s)\}.\]
%Let $\tilde{\mathcal{T}}=$\{$\tau \mid \tau\in enabled(s) \quad \wedge \quad \tau$ ranks first in $enabled(s)$  for all $s\in S$\}. Let $\tilde{G} = (S,\tilde{\mathcal{T}})$.
 \end{Definition}

We can see that this $\tilde{G}$ is formed according to the on-the-fly schedule, in which we always schedule the active process with the smallest rank. Now, we can present the main theorem, which guarantees the completeness and soundness of the on-the-fly schedule.

\setcounter{theorem}{0}
\begin{theorem}
\label{theorem1}
Given an execution $\pi$ in $G$ from a global initial state $\sigma_0$ to a deadlocked global state $\sigma$, there exists an execution $T$ from $\sigma_0$ to $\sigma$ in $\tilde{G}$ such that $\lvert T\rvert = \lvert \pi \rvert$. And vice versa.
\end{theorem}
To prove the above theorem, we introduce some notions first.
%Assuming transition system is \emph{action-deterministic}, \emph{i.e.} for any state $s$ and action $act$, there is at most one outgoing transition from $s$ with action $act$.
An \emph{independent} relation $I\in Act \times Act$ is a relation, satisfying the following two conditions:\\
for any state $s \in S$,  with $\alpha,\beta \in enabled(s)$ and $\alpha \neq \beta$,
\begin{itemize}
%\item \emph{Enabledness} If $\alpha,\beta \in enabled(s)$ then $\alpha\in enabled(\beta(s))$.
%\item \emph{Commutativity} $\alpha,\beta\in enabled(s)$ then $\alpha(\beta(s))=\beta(\alpha(s))$.
\item \emph{Enabledness}     $\alpha\in enabled(\beta(s))$ , $\beta \in enabled(\alpha(s))$.
\item \emph{Commutativity}  $\alpha(\beta(s))=\beta(\alpha(s))$.

\end{itemize}
Recall that $\alpha(s)$ denotes the unique $\alpha$ successor of $s$, \emph{i.e.} if $ s\overset{\alpha}{\rightarrow} s'$ holds, then $s'=\alpha(s)$. The dependency relation $D$ is the complement of $I$, \emph{i.e.}, $D = Act \times Act - I$.

The method we constructing a subgraph $\tilde{G}$  from a graph $G$ actually falls into the \emph{ample set} method proposed in  \cite{Clarke:2000:MC:332656}, which expands only a part of the transitions at each state, for a path not considered by the method, there is an equivalent path with respect to the specification considered. Among the four conditions \textbf{C0}-\textbf{C3} for selecting $ample(s)\subseteq enabled(s)$, the first two are as follows:\\
$\mathbf{C0} \quad ample(s)=\emptyset$ if and only if $enabled(s)=\emptyset$.\\
$\mathbf{C1}$\quad Let $s_0\overset{\alpha_0}{\rightarrow}s_1,\dots,\overset{\alpha_{n}}{\rightarrow}s_n\overset{\alpha_{n+1}}
{\rightarrow}t$ be a finite execution fragment, if $\alpha_{n+1}$ depends on $\beta\in ample(s_0)$, then there exists an $\alpha_i\in ample(s_0)$, where $0\leq i < n+1$, \emph{i.e.}, along every execution in the full state graph $G$ that starts at $s$, an action appears in the execution fragment starts at $s$ which is dependent on an action in $ample(s)$ cannot be executed without an action in $ample(s)$ occurring first.

 \textbf{C2} makes sure that: when $ample(s)\neq enabled(s)$, the actions in $ample(s)$ do not change the label of states with respect to the verifying properties. Here the property we concerned with is deadlock-reachability. Since we commute independent actions by applying \emph{commutativity} of independent relation, we do not need \textbf{C2}.
%Hence all we need is that for an action $\alpha\in ample(s)$ with $ample(s)\neq enabled(s) \wedge s_1\overset{\alpha}{\rightarrow}s_2$, if $s_1$ is deadlock-reachable, then $s_2$ is deadlock-reachable.
\textbf{C3} ensures that a cycle in the reduced graph needs to satisfy some requirements. Owing to the acyclicity of the state space in out context, we do not need \textbf{C3}.


In our circumstance, we define $ample(s)$ as following:
%$$ample(s) =\left\{
% \begin{array}{ll}
%    \{B\} & \textrm{if $\exists s'\in S, s\overset{B}{\rightarrow}s'$} ; \\
%    \{SR\} & \textrm{else if $\exists s'\in S, s\overset{SR}{\rightarrow}s'  \wedge SR$}\textrm{ ranks first in $eanbled(s)$}.
% \end{array}
%\right. $$
$$ample(s) =\left\{
 \begin{array}{ll}
    \{B\} & \textrm{if $B\in enabled(s)$} ; \\
    \{SR\} & \textrm{else if $SR\in enabled(s)  \wedge SR$}\textrm{ ranks first in $enabled(s)$}.
 \end{array}
\right. $$
%for global state $s$ in $G$ is the global B act, or the one ranks first in $enabled(s)$. Now we can turn to the proof of Theorem \ref{theorem-1}.
Note that for a state $s\in S$, if $enabled(s)\neq \emptyset$, $\lvert ample(s)\rvert = 1$, \emph{i.e.}, $ample(s)$ has only one element. Hence, $C_0$ surely holds.

To check whether \textbf{C1} holds on the full state graph generated by our schedule algorithm, we first introduce some properties of the full state graph. Clearly, according to the definition of parallel composition, only $SR$ actions can be enabled simultaneously at a global state, and the $SR$ actions enabled at a same state are independent.
%Note that in the full state graph, both $SR$ and $B$ actions could not disable other actions, and for actions $\alpha,\beta\in enabled(s)$, $\langle\alpha,\beta\rangle\in I$, which comes from the observation that
%and if there is an execution $\pi$ set $B\prec_{eb}\alpha$, \emph{i.e.}, $B$ executes before another action $\alpha$, then in all executions this $B\prec_{eb}\alpha$. And if in $\pi$, $\alpha\prec_{eb}B$, then in all execution fragment $\alpha\prec_{eb}B$.  This is ensured by MPI's barrier semantics.
%Here we check \textbf{C1}.
So, given a execution fragment $\pi=s_0\overset{\alpha_0}{\rightarrow}s_1\dots,\overset{\alpha_{j-1}}{\rightarrow}s_j\overset{\alpha_j}{\rightarrow}s_{j+1}$ starting from $s_0\in S$, $\alpha_j$ depends on an action $\beta\in ample(s_0)$. We want to prove that there exists a $\alpha_k$, where $0 \leq k < j$, and $\alpha_k \in ample(s_0)$.  Recall the definition of dependent relation $D$, we know that $\alpha_j$ and $\beta$ should meet one of the following cases:
\begin{enumerate}
  \item $\nexists s\in S$ such that $\alpha_j,\beta\in enabled(s)$;
  \item for any state $s\in S$, if $\alpha_j,\beta\in enabled(s)$, then $\alpha_j\not\in enabled(\beta(s))$ or $\beta \not\in enabled(\alpha_j(s))$, \emph{i.e.}, either $\alpha_j$ disables $\beta$ or $\beta$ disables $\alpha_j$;
  \item for any state $s\in S$, if $\alpha_j,\beta\in enabled(s)$ and $\alpha_j\in enabled(\beta(s)) \wedge \beta \in enabled(\alpha_j(s))$, then $\alpha_j(\beta(s)) \neq \beta(\alpha_j(s))$, \emph{i.e.}, $\alpha_j$ and $\beta$ are not commutative.
\end{enumerate}

Because only $SR$ actions can be enabled simultaneously at a global state, both case 2 and case 3 cannot hold under our context. Therefore, only case 1 holds for the state graph generated by our method, \emph{i.e.}, $\alpha_j$ and $\beta$ should not be both enabled at any state. Based on this result, we can get \textbf{C1} holds in our context by contradiction. Assume that $\{\alpha_0\dots\alpha_{j-1}\}\cap ample(s_0) = \emptyset$ holds for the execution $\pi$. Because $\beta$ is enabled at $s_0$, $\alpha_0$ and $\beta$ are independent, hence $\beta$ is also enabled at $s_1$. In addition, $\alpha_1$ is also enabled at $s_1$ and $\alpha_1 \neq \beta$, so $\alpha_1$ and $\beta$ are also independent. In the same way, we can get that each $\alpha_i\ ( 0\leq i < j)$ and $\beta$ are independent. Thus, by using commutativity,  we can get $\beta$ and $\alpha_j$ are both enabled at $s_j$, which violates \mbox{case 1}. Hence, the condition \textbf{C1} holds.

\begin{proof}
One direction, because $\tilde{G}$ is a subgraph of $G$, the execution $T$ from $\delta_0$ to $\delta$ in $\tilde{G}$ is also an execution from $\delta_0$ to $\delta$ in $G$, hence we got an execution $\pi = T$, and $\lvert T \rvert = \lvert \pi \rvert$.

The other direction is a little more complex. The basic idea is to construct a corresponding execution in the subgraph gradually based on the $ample$ set of each state passed in $\pi$.

Let $\pi$ be an execution in $G$ from $\delta_0$ to $\delta$. We construct a finite sequence of executions $\pi_0,\pi_1,\dots,\pi_n$, where $\pi_0 = \pi$ and $n=\lvert \pi \rvert$. %Each execution $\pi_i$ is decomposed into two execution fragments, $\eta_i$ and $\theta_i$, where $\eta_i$ is of length $i$.
Each execution $\pi_i$ is constructed based on the before execution $\pi_{i-1}$. For example, $\pi_1$ is constructed from $\pi_0$, \emph{i.e.}, $\pi$, according to the first action execution in $\pi$. Thus, we want to prove that the last execution $\pi_n$ is an execution in the subgraph, and shares the same first and last states with $\pi$. We can prove it by presenting the construction method of each step. We decompose each $\pi_i$ into two execution fragments, \emph{i.e.}, $\pi_i = \eta_i\circ\theta_i$, where $\eta_i$ is of length $i$ and $\eta_{i}\circ\theta_{i}$ is the concatenation of the two execution fragments.

Assuming that we have constructed $\pi_0,\dots,\pi_i$, we now turn to construct $\pi_{i+1} = \eta_{i+1}\circ\theta_{i+1}$. Let $s_0$ be the last state of the execution fragment $\eta_i$ and $\alpha$ be the first action of $\theta_i$. Note that $s_0$ is also the first state of the execution fragment $\theta_i$, \emph{i.e.},
$$\theta_i = s_0 \overset{\alpha_0 = \alpha}{\longrightarrow}s_1\overset{\alpha_1}{\longrightarrow}s_2\overset{\alpha_2}{\longrightarrow}\dots s_{\lvert \theta_i \rvert}$$
There are two cases:\\
   \textbf{A.} $\alpha\in ample(s_0)$. Then $\eta_{i+1} = \eta_{i}\circ (s_0\overset{\alpha}{\rightarrow}{\alpha(s_0)})$ and $\theta_{i+1}=s_1\overset{\alpha_1}{\longrightarrow}s_2\overset{\alpha_2}{\longrightarrow}\dots s_{\lvert \theta_i \rvert}$.\\ %which is $\theta_i$ without it's first state and action.\\
    \textbf{B.} $\alpha\not\in ample(s_0)$.  Note that $s_{\lvert \theta_i \rvert} = \sigma$ is a deadlock state, hence no action can be enabled at $\sigma$. Therefore, for any action $\beta\in ample(s_0)$, some actions that appear in $\theta_i$ must be dependent on $\beta$. The reason is: if all the actions that appears in $\theta_i$ is independent of $\beta$, then all the actions in $\theta_i$ cannot disable $\beta$, hence $\beta$ would be enabled at $s_{\lvert \theta_i \rvert} = \sigma$, which violates the premiss that $\sigma$ is a deadlock state.

%Hence $\beta$ is dependent with some $\alpha_j$.
%By $\mathbf{C1}$, there must be a  $\beta'\in ample(s_0)$ must occur first in $\theta_i$, hence there exists $0<k < j$, such that $\alpha_k =\beta'$ and $\alpha_0\alpha_1\alpha_2\dots\alpha_{k-1}$ is a sequence of actions independent with $\beta'$. Then there is an execution $\xi = s_0\overset{\beta'}{\rightarrow}\beta'(s_0)\overset{\alpha=\alpha_0}{\longrightarrow}\beta'(s_1)\overset{\alpha_1}{\longrightarrow}\dots \overset{\alpha_{k-1}}{\longrightarrow}\beta'(s_k)\overset{\alpha_{k+1}}{\longrightarrow}s_{k+2}\overset{\alpha_{k+2}}{\longrightarrow}\dots\overset{\alpha_{\lvert \theta_i \rvert -1 }}{\longrightarrow}s_{\lvert \theta_i \rvert}$ in $G$. That is, by using the commutativity condition of dependent relation $k$ times, we get this execution from $\theta_i$. Note that $\beta' = \alpha_k$, hence $\beta'(s_k) = s_{k+1}$.
Therefore, for any action $\beta$ in $ample(s_0)$, we can find an action $\alpha_j$ that appears in $\theta_i$, and $\alpha_j$ depends on $\beta$. According to \textbf{C1}, there must exist an action $\beta' \in ample(s_0)$, such that $\beta'$ occurs before $\alpha_j$. Because there may exist multiple actions that are in $ample(s_0)$ and occur before $\alpha_j$, we take the first one, say $\alpha_k$ and $\alpha_k \in ample(s_0)$. So, $\alpha_k$ is the first one among the elements of $ample(s_0)$ that occur in $\theta_i$. Clearly, the actions before $\alpha_k$, \emph{i.e.}, $\alpha_0, ..., \alpha_{k-1}$, are independent with $\alpha_k$. Hence, we can construct the following execution by using the commutativity condition $k$ times: \\
 $\xi = s_0\overset{\alpha_k}{\rightarrow}\alpha_k(s_0)\overset{\alpha=\alpha_0}{\longrightarrow}\alpha_k(s_1)\overset{\alpha_1}{\longrightarrow}\dots \overset{\alpha_{k-1}}{\longrightarrow}\alpha_k(s_k)\overset{\alpha_{k+1}}{\longrightarrow}s_{k+2}\overset{\alpha_{k+2}}{\longrightarrow}\dots\overset{\alpha_{\lvert \theta_i \rvert -1 }}{\longrightarrow}s_{\lvert \theta_i \rvert}$.


In this case $\eta_{i+1}=\eta_i \circ (s_0\overset{\alpha_k}{\rightarrow}\alpha_k(s_0))$ and $\theta_{i+1}$ is the execution fragment that is obtained from $\xi$ by removing the first transition $s_0\overset{\alpha_k}{\rightarrow}\alpha_k(s_0)$.

Clearly, $\pi_i$ and $\pi_{i+1}$ share the same last state. So, $\pi_0 = \delta$ and $\pi_{n}$ share the same last state of the execution, namely $\pi_{n}$ is also an execution from $\delta_0$ to $\delta$ in $G$. In addition, according to the construction procedure, $\lvert \pi \rvert = \lvert \pi_{ n}\rvert$ holds. Most importantly, in execution $\pi_{n}$, for any $0\leq j< n$, such that $s_j\overset{\alpha_j}{\longrightarrow}s_{j+1}$, $\alpha_j\in ample(s_j)$ holds. Therefore, $\pi_{n}$ is also an execution from $\delta_0$ to $\delta$ in $\tilde{G}$, and we take this execution as $T$.\Qed
\end{proof}



To prove the correctness and soundness of our lazy matching algorithm, we need to deal with wildcard receives. Hence the rules of parallel composition of transition systems need to be refined. Instead of redefine $match$ to make it work with wildcard receives, we make a new rule for matched send and wildcard receives, to distinct it with source specific receives.
\begin{itemize}
\item for matched actions $\alpha,\beta \in H=\{s,r_{*}\}$ in distinct processes, where $r_*$ is the wildcard receive:
 $$\frac{s_i\overset{\alpha}{\rightarrow_i}s'_i \quad\wedge\quad s_j\overset{\beta}{\rightarrow_j}s'_j  \quad\wedge\quad match(\alpha, \beta)}{\langle s_1,\dots,s_i,\dots ,s_j,\dots s_n\rangle\xrightarrow{SR_*}{\langle s_1,\dots,s'_i,\dots ,s'_j,\dots s_n\rangle}}$$ here $match(\alpha,\beta)$ if and only if $\alpha= s \wedge \beta=r_* $,  $dest(\alpha)=j$, and $dest(\beta)=ANY$, $SR_*$ is the compositional global action of $s$ and $r_*$.
\end{itemize}
We also need to redefine the subgraph $\tilde{G}$ because we have a new kind of global transitions.


 \begin{Definition}
%\{\tau\mid \tau \in subtrans(s),  s\in S\}$
 Let $\tilde{\mathcal{T}}= \underset{s\in S}{\bigcup} subtran(s)$ , where $subtrans(s)$ is defined as:
 {\small
$$subtran(s) =\left\{
 \begin{array}{ll}
    \{s\overset{B}{\rightarrow}B(s)\} & \textrm{if $B \in enabled(s)$} ; \\
    \{s\overset{SR}{\rightarrow}SR(s)\} & \textrm{else if $SR \in enabled(s) \wedge$}
         SR\ \textrm{ranks first in $enabled(s)$}; \\
    \{s\overset{act}{\rightarrow}act(s)\}   & \textrm{else if $act\in enabled(s)$}.
  \end{array}
\right. $$}\\
  Let $\tilde{G_*} = (S,\tilde{\mathcal{T}})$, which is a subgraph of the full state graph.
 \end{Definition}

Clearly, we can see that $\tilde{G_*}$ is the subgraph we formed according to the on-the-fly schedule plus lazy matching. Accordingly, we define $ample(s)$ as:
$$ample(s) =\left\{
 \begin{array}{ll}
    \{B\} & \textrm{if $B\in enabled(s)$} ; \\
    \{SR\} & \textrm{else if $SR\in enabled(s)  \wedge SR$}\textrm{ ranks first in $enabled(s)$};\\
    enabled(s) & \textrm{other}.
 \end{array}
\right. $$

And the following theorem addresses the correctness and soundness of lazy matching algorithm:

\begin{theorem}
\label{theorem2}
Given any execution $\pi$ in $G$ from a global state $\sigma_0$ to a deadlocked global state $\sigma$, there exists an execution $T$ from $\sigma_0$ to $\sigma$ in $\tilde{G_*}$ such that $\lvert T\rvert = \lvert \pi \rvert$. And vice versa.
\end{theorem}

To prove theorem \ref{theorem2}, we first check the conditions \textbf{C0} and \textbf{C1}. Clearly, \textbf{C0} holds. To check \textbf{C1}, we should point out that in the new global state graph, an action $SR\in enabled(s)$ is independent with the rest actions in $enabled(s)$. In addition, only $SR_*$ can disable other $SR_*$ actions, which is ensured by the semantics of wildcard receives. %Now we turn to check \textbf{C1}.
Same as before, given a execution fragment $\pi=s_0\overset{\alpha_0}{\rightarrow}s_1\dots,\overset{\alpha_{j-1}}{\rightarrow}s_j\overset{\alpha_j}{\rightarrow}s_{j+1}$ starting from $s_0\in S$, $\alpha_j$ depends on an action $\beta \in ample(s_0)$. We want to prove that there exists a $\alpha_k$, where $0 \leq k < j$, and $\alpha_k \in ample(s_0)$.
%Given a execution fragment $\pi=s_0\overset{\alpha_0}{\rightarrow}s_1\dots,\overset{\alpha_{j-1}}{\rightarrow}s_j\overset{\alpha_j}
%{\rightarrow}s_{j+1}$ starts at $s_0\in S$, assume that $\langle \alpha_j, \beta\rangle\in D$, where $\beta\in ample(s_0)$. Recall the definition of dependent relation $D$, we know that $\alpha_j$ and $\beta$ should meet one of the following conditions:
%\begin{enumerate}
%  \item $\nexists s\in S$ such that $\alpha_j,\beta\in enabled(s)$;
%  \item for any state $s\in S$, if $\alpha_j,\beta\in enabled(s)$, then $\alpha_j\not\in enabled(\beta(s))$ or $\beta \not\in enabled(\alpha_j(s))$, \emph{i.e.} either $\alpha_j$ disables $\beta$ or $\beta$ disables $\alpha_j$;
%  \item for any state $s\in S$, if $\alpha_j,\beta\in enabled(s)$ and $\alpha_j\in enabled(\beta(s)) \wedge \beta \in enabled(\alpha_j(s))$, then $\alpha_j(\beta(s)) \neq \beta(\alpha_j(s))$, \emph{i.e.}, $\alpha_j$ and $\beta$ are not commutative.
%\end{enumerate}
%We discuss all the cases of $\alpha_j$:
%\begin{enumerate}
%  \item $\alpha_j\in ample(s_0) \subseteq enabled(s_0)$. Clearly, \textbf{C1} holds if $ample(s_0) = enabled(s_0)$.
%%   in this case, $\alpha_j$ itself is a occurrence of an element of $ample(s_0)$;
%  \item $\alpha_j\in enabled(s_0) \setminus ample(s_0)$, then $ample(s_0)\neq enabled(s_0)$, hence we can get $ample(s_0)= \{SR\}$. According to the observation, $SR$ is independent with each of the rest actions in $enabled(s_0)$, so $\alpha_j$ and $SR$ are independent. Therefore, it is a contradiction, thus this case never happens.
%  \item $\alpha_j\not\in enabled(s_0)$. If $ample(s_0) = enabled(s_0)$, \textbf{C1} clearly holds. Now we discuss $ample(s_0) \neq enabled(s_0)$, \emph{i.e.}, $ample(s_0) = \{SR\}$, thus $\beta$ is $SR$. And, for an $SR$ action, the dependent relation can only be one case, \emph{i.e.}, $\nexists s\in S$ such that $\alpha_j,\beta\in enabled(s)$.
%  Because $SR$ will never be disabled by any other action, same as the idea for proving \textbf{C0} for the case without wildcard receives, we can prove that $\beta$ occurs before $\alpha_j$.
%\end{enumerate}
We discuss the two cases of $ample(s_0)$:
\begin{enumerate}
  \item $ample(s_0) = enabled(s_0)$. Clearly, \textbf{C1} holds.
%   in this case, $\alpha_j$ itself is a occurrence of an element of $ample(s_0)$;
  \item $ample(s_0) \neq enabled(s_0)$. Thus, $ample(s_0) = \{SR\}$ and $\beta = SR$. %It is clear that $\alpha_j$ should not be $SR$.
We then discuss two cases: 1) $\alpha_j\in enabled(s_0) \setminus ample(s_0)$, according to the observation, $SR$ is independent with each of the rest actions in $enabled(s_0)$, so $\alpha_j$ and $SR$ are independent. Therefore, it is a contradiction, thus this case never happens. 2) $\alpha_j\not\in enabled(s_0)$. For an $SR$ action, the dependent relation of it can only be one case, \emph{i.e.}, $\nexists s\in S$ such that $\alpha_j,\beta\in enabled(s)$.
  Because $SR$ will never be disabled by any other action, same as the idea for proving \textbf{C1} for the case without wildcard receives, we can prove that $\beta$ occurs before $\alpha_j$.
\end{enumerate}
In total, we can get that \textbf{C1} holds on the new state graph.

\begin{proof}
We have concluded that the condition \textbf{C0} and \textbf{C1} still holds in the new full state graph. Hence, the procedure of the proof for theorem 2 is basically the same with that of theorem 1.
\Qed
\end{proof}


==> mpiklee-lastest - extended/related.tex <==
% !TEX root = main.tex
%
\section{Related Work}
\label{Sec: Related}

There are already some existing work for improving the reliability of MPI programs \cite{Gopalakrishnan:2011:FAM:2043174.2043194}. Generally, they often fall into one of the following two categories: debugging and testing methods, and verification methods.

Debugging and testing tools often scale well, but depend on concrete inputs to run MPI programs, expecting to find or locate bugs. Debugging tools such as TotalView \cite{TotalView} and DDT \cite{DDT} are often effective when the bugs can be replayed consistently. Whereas, for MPI programs, reproducing a concurrency bug caused by non-determinism is itself a challenging problem. Another kind of tools, such as Marmot \cite{KrammerBMR03}, the Intel Trace Analyzer and Collector \cite{ita} and MUST \cite{Hilbrich:2012:MRE:2388996.2389037}, intercept MPI calls at runtime and record the running information of an MPI program, and check runtime errors, deadlock or analyze performance bottlenecks based on the recorded runtime information. These tools often need to recompile or relink MPI programs, and also depend on the inputs and the scheduling of each running.

Another line of tools are verification tools. Dynamic verification tools, such as ISP \cite{ppopp-VakkalankaSGK08} and DAMPI \cite{Vo:2010:SDD:1884643.1884681}, provide a coverage guarantee over the space of MPI non-determinism. When two or more matches of a non-deterministic operation, such as wildcard receive is detected, the program will be re-executed, and each running using a specific match. Hence, these tools can find the bug relying on a particular choice when non-deterministic operations are encountered, but also depend on the inputs that are fed to run the program. TASS \cite{TASS} tackles the limitation by using symbolic execution to reason about all the inputs of an MPI program, but its feasibility is limited by the simple MPI model used, which is justified in Section \ref{subSec:ee}. There are few static analysis work for MPI program. Greg proposes in \cite{DBLP:conf/cgo/Bronevetsky09} a novel data flow analysis notion, called \emph{parallel} control flow graph (pCFG), which can capture the interaction behavior of an MPI program with arbitrary number of processes. Based on pCFG, some static analysis activities can be carried out. %such as getting the communication topology of an MPI program. 
However, the static analysis based on pCFG is hard to be automated.

Compared with the existing work, \mpise{} symbolically executes MPI programs and uses an on-the-fly scheduling algorithm to handle non-determinism, and provides the coverage guarantee on both input and non-determinism. In addition, \mpise{} uses a realistic MPI library, \emph{i.e.}, TOMPI \cite{Demaine97athreads-only}, to be the MPI model used. Therefore, more realistic MPI programs can be analyzed automatically by \mpise{}, without modifying the programs manually. Furthermore, since the MPI library and the symbolic executor are loosely coupled by hooking the library, it is not hard to switch to another implementation of MPI library to improve the precision and the feasibility of symbolic execution.

